A Marginal Dimension of a Weakly Diluted Quenched m-Vector Model

We calculate a marginal order parameter dimension $m_c$ which in a weakly diluted quenched $m$-vector model controls the crossover from a universality class of a ``pure'' model ($m>m_c$) to a new universality class ($m<m_c$). Exploiting the Harris criterion and the field-theoretical renormalization group approach allows us to obtain $m_c$ as a five-loop $\epsilon$-expansion as well as a six-loop pseudo-$\epsilon$ expansion. In order to estimate the numerical value of $m_c$ we process the series by precisely adjusted Pad\'e--Borel--Leroy resummation procedures. Our final result $m_c=1.912\pm0.004<2$ stems from the longer and more reliable pseudo-$\epsilon$ expansion, suggesting that a weak quenched disorder does not change the values of $xy$-model critical exponents as it follows from the experiments on critical properties of ${\rm He}^4$ in porous media.

==> brlccod.tex <==
\uccode'240='200 \lccode'240='240 %a
\uccode'241='201 \lccode'241='241 %b
\uccode'242='202 \lccode'242='242 %v
\uccode'243='203 \lccode'243='243 %g
\uccode'244='204 \lccode'244='244 %d
\uccode'245='205 \lccode'245='245 %e
\uccode'246='206 \lccode'246='246 %zhe
\uccode'247='207 \lccode'247='247 %z
\uccode'250='210 \lccode'250='250 %i
\uccode'251='211 \lccode'251='251 %short i
\uccode'252='212 \lccode'252='252 %k
\uccode'253='213 \lccode'253='253 %l
\uccode'254='214 \lccode'254='254 %m
\uccode'255='215 \lccode'255='255 %n
\uccode'256='216 \lccode'256='256 %o
\uccode'257='217 \lccode'257='257 %p
\uccode'340='220 \lccode'340='340 %r
\uccode'341='221 \lccode'341='341 %s
\uccode'342='222 \lccode'342='342 %t
\uccode'343='223 \lccode'343='343 %u
\uccode'344='224 \lccode'344='344 %f
\uccode'345='225 \lccode'345='345 %kh
\uccode'346='226 \lccode'346='346 %ts
\uccode'347='227 \lccode'347='347 %ch
\uccode'350='230 \lccode'350='350 %sh
\uccode'351='231 \lccode'351='351 %shch
\uccode'352='232 \lccode'352='352 %hard sign (yer)
\uccode'353='233 \lccode'353='353 %y (yery)
\uccode'354='234 \lccode'354='354 %soft sign (yerik)
\uccode'355='235 \lccode'355='355 %reverse e
\uccode'356='236 \lccode'356='356 %yu
\uccode'357='237 \lccode'357='357 %ya
\uccode'361='360 \lccode'361='361 %yo
\uccode'363='362 \lccode'363='363 %g (ukrainian hard g)
\uccode'365='364 \lccode'365='365 %ye (ukrainian ye)
\uccode'367='366 \lccode'367='367 %i (ukrainian i)
\uccode'371='370 \lccode'371='371 %yi (ukrainian yi)
%
\uccode'200='200 \lccode'200='240 %A
\uccode'201='201 \lccode'201='241 %B
\uccode'202='202 \lccode'202='242 %V
\uccode'203='203 \lccode'203='243 %G
\uccode'204='204 \lccode'204='244 %D
\uccode'205='205 \lccode'205='245 %E
\uccode'206='206 \lccode'206='246 %ZH
\uccode'207='207 \lccode'207='247 %Z
\uccode'210='210 \lccode'210='250 %I
\uccode'211='211 \lccode'211='251 %short I
\uccode'212='212 \lccode'212='252 %K
\uccode'213='213 \lccode'213='253 %L
\uccode'214='214 \lccode'214='254 %M
\uccode'215='215 \lccode'215='255 %N
\uccode'216='216 \lccode'216='256 %O
\uccode'217='217 \lccode'217='257 %P
\uccode'220='220 \lccode'220='340 %R
\uccode'221='221 \lccode'221='341 %S
\uccode'222='222 \lccode'222='342 %T
\uccode'223='223 \lccode'223='343 %U
\uccode'224='224 \lccode'224='344 %F
\uccode'225='225 \lccode'225='345 %KH
\uccode'226='226 \lccode'226='346 %TS
\uccode'227='227 \lccode'227='347 %CH
\uccode'230='230 \lccode'230='350 %SH
\uccode'231='231 \lccode'231='351 %SHCH
\uccode'232='232 \lccode'232='352 %Hard sign (Yer)
\uccode'233='233 \lccode'233='353 %Y (Yery)
\uccode'234='234 \lccode'234='354 %Soft sign (Yerik)
\uccode'235='235 \lccode'235='355 %Reverse e
\uccode'236='236 \lccode'236='356 %YU
\uccode'237='237 \lccode'237='357 %YA
\uccode'360='360 \lccode'360='361 %YO
\uccode'362='362 \lccode'362='363 %G (ukrainian hard G)
\uccode'364='364 \lccode'364='365 %YE (ukrainian YE)
\uccode'366='366 \lccode'366='367 %I (ukrainian I)
\uccode'370='370 \lccode'370='371 %YI (ukrainian YI)

